The symplectic geometry of the three-body problem

A book, concerning the classical restricted three body problem, and the approach to this old conundrum coming from the modern methods of symplectic and contact geometry. It is split into Part I (theoretical aspects), and Part II (practical aspects). The main themes are Floer theory, contact topology, symplectic dynamics, and astrodynamics (with a view towards space mission design).

==> backup_with_acknowledgments.tex <==
To Helmut Hofer, for being a constant inspiration and a great mentor; this work would not exist if it were not for your guidance. To Chris Wendl, my former PhD supervisor, for the support throughout the years. To Kai Cieliebak, a great mathematician and mentor, and a greater person.
To my collaborators Fabio Gironella, Jonathan Bowden, Zhengyi Zhou, Oleg Lazarev and Thomas Massoni, my extended family of incredibly talented people, for keeping me on my toes with so much math. To Peter Sarnak, for great mathematical insights and for pushing me in the right directions. To Richard Montgomery, for great feedback and for listening to my (sometimes wacky) ideas. To Daniel Scheeres, for the open-mindedness to new ideas; let us hope for productive years of work to come. To Ed Belbruno, a living legend, you not only saved the HITEN mission, but also the confidence in my artistic work. To Peter Albers, for constant enthusiasm, supporting my work, and teaching me how to run a research group by setting the example. To Sergei Tabachnikov, for passing to me his infectious enthusiasm for billiards. To László Székelyhidi, for the music we have shared, and the music we \emph{will} share. To Peter Ozváth, my enthusiastic partner in all-things-cello crimes, thank you for keeping my fingers on my cello. To Matteo Parisi, for wonderful hours of Prokofiev and Schubert together. To Lei Zhao, for the support and feedback in the early stages of this work. To  Connor Jackman, for helping me shape the way I think about celestial mechanics. To Jordan Berman, a creative genius, for believing in that I have a story to tell. To Karen Uhlenbeck and Bob Williams, for inspiring me with so many stories of their own, and for gifting me Atiyah's complete works, now one of my most cherished possessions. To Bill Goldman, the nicest person I have ever met, for so much math and drinks and food. To Jo Nelson, for the sheer amount of fun I have every time we get together; I hope next time I get stuck in Houston we will indeed go for beers. To Julian Chaidez, Princeton would have been a duller place without you, man. To Sobhan Seyfaddini, for showing me that mathematical life can be only continuous, and still beautiful, and helping me through the very painful process of applying to an ERC grant. To Michael Hutchings, for interest in this work, and gread reading recommendations. To Vini Ramos, for the enthusiasm and the pleasure I get when working together. To Georgios Dimitroglou Rizell, for making my time in Sweden so enjoyable and keeping my Lagrangians tamed. To Richard Siefring, for all the steak, the whisky, and the intersection theory. To Ezequiel Maderna, Alejandro Passeggi and Rafael Potrie, my fellow uruguayan colleagues, thank you for helping me leave a grain of sand in the uruguayan mathematical community. To my students Arthur Limoge, Favio Pir\'an and Francesco Ruscelli, for keeping me busy answering good questions. To my music group, Lay Kodama, Kin Lam, Will Berdanier, Franca Hoffmann, Jumpei Satomi, Philip Zupancic, Jozefien Vanherpe; you guys are family. 

To my mother, Gabriela López, and my brother, Julián Moreno, for keeping my feet on this Earth and not flying around the Jupiter--Europa system; I could not have done this work without you. %Last but not least, to Svitlana Mayboroda, my partner, for constant inspiration; I am  grateful for sharing my life with you. 
